Reversible Computation in Petri Nets

Reversible computation is an unconventional form of computing that extends the standard forward-only mode of computation with the ability to execute a sequence of operations in reverse at any point during computation. As such, in this thesis we propose a reversible approach to Petri nets by introducing machinery and associated operational semantics to tackle the challenges of the main forms of reversibility. Our proposal concerns a variation of cyclic Petri nets, called Reversing Petri Nets (RPNs) where tokens are persistent and distinguished from each other by an identity. An immediate extension of the original model includes allowing multiple tokens of the same base/type to occur in a model. Specifically, we explore the individual token interpretation where one distinguishes different tokens residing in the same place by keeping track of where they come from. We also propose the collective token interpretation, as the opposite approach to token ambiguity, which considers all tokens of a certain type to be identical, disregarding their history during execution. Both of the proposed models of RPNs (with single or multi tokens) implement the notion of uncontrolled reversibility, meaning that it specifies how to reverse an execution and allows to do so freely, yet it places no restrictions as to when and whether to prefer backward execution over forward execution or vice versa. In this respect, a further aim is to control reversibility by extending our formal semantics where transitions are associated with conditions whose satisfaction allows the execution of transitions in the forward/reversed direction.

==> 2.ReversibleComputation.tex <==
\subsection{Overview}
%computers are forward-only
Mechanical Computing essentially dates back to the 1800s followed by Electronic Computing starting at least six decades ago and ever since both of them have been supporting and enhancing all aspects of our lives ~\cite{perumalla}. Current computer technology, which operates in the de-facto forward-only mode,  yields various risks and costs due to modern society's critical dependence. Forward-only computing  has been extensively researched, developed  and analysed in academia, industry and government across the globe. For the entire history of computing, computers have been based on the irreversible mode of computation since in the concurrent setting computers are non-deterministic in both the forward and backward direction of execution. Forward direction is the standard kind of execution whereas backward direction is the ability to go back to previous states by undoing previously executed actions. 

% which means they are non-deterministic
Since current technology is not invertible it leads to  loss of information where previous states cannot be recovered from the current state. It follows an irreversible computation paradigm where ordinary computer chips do not qualify for reversible logic gates. For example, a simple standard operation, like the logical AND, illustrates that given the output 0 it is impossible to determine the input values as one of the 1 and 0, 0 and 1 or 0 and 0 ~\cite{RCwille}. Therefore, such logically irreversible operations lack determinism because the partial function that maps each machine state onto its successor generates more than one inverse values.  

%RC is the ability to have backward determinism
This entails that, if there is a logic gate that generates an output from a given input, the gate is reversible only when there is an inverse operation that performs a bijective transformation of its local configuration space. Crucially, the ability to have two-way determinism requires an one-to-one mapping, where each input produces a unique output. These bijective reversible operations have at most one previous configuration giving the ability to uniquely identify the forward or backward state at any point of the execution. Such backward deterministic systems are the foundations of an alternative computation paradigm, called Reversible Computation. Therefore, a computation is logically reversible if it is always possible to efficiently reconstruct the previous state of the computation from its current state.


% Thus, RC moves back and forth in states
Reversible computation is an emerging paradigm that extends the standard forward-only mode of computation by allowing one to execute programs in the backward direction as effortlessly as it can be executed in the standard forward direction. In particular, individual operations become time reversible that can easily and exactly be reversed, or undone at any point of the execution. Computer scientists believe that Reversible Computation is a very unconventional but promising form of computing, which is able to deliver novel computing devices and software. More importantly, reversibility is emerging as one of the most exciting new dimensions in computing for the future, positioned for inevitable progress and expansion in the coming decades. 

\subsection{Motivation}
%Physics are already Reversible so should computing 
Reversible computing combines thermodynamics and information theory in order to reflect physical reversibility one of the fundamental microscopic physical properties of Nature. Since all successful fundamental physical theories share the property of reversibility, future computing should also follow rather trivially certain basic facts of fundamental physics. Such properties can be effectively used in computing in order to create an interface between computation and the laws of physics where logical reversibility implements physical reversibility~\cite{RCA-survey}.  

%landauer notes  that physics are reversible 
Back to the 1960's, three foundational studies of information lossless computations made their appearance. Having different motivations, Huffman studied finite state machines that do not erase information~\cite{Huffman},  Lecerf studied the theoretical properties of reversible Turing machines~\cite{lecerf} and Landauer studied the thermodynamics of reversible logics. Of these  studies Landauer's work is the most prominent, but the other two have laid the foundation of the theoretical study of reversible computing.

Physicist Rolf Landauer was the first to argue the relation between thermodynamics and the irreversible character of conventional computers. Specifically, reversible computation originated in the 60's when Landauer published a paper titled ``Irreversibility and Heat Generation in the Computing Process"~\cite{Landauer}, where he attempted to apply the most fundamental, reversible laws  of physics to digital computers.  Landauer's key insight follows directly as an immediate logical consequence of our most thorough, battle-tested understanding of fundamental physics. He noted that, while classical mechanics and quantum mechanics are fundamentally reversible~\cite{Structural} by obeying the laws of motion, their logical state often evolves irreversibly since it is not backward deterministic. This means that since all of the fundamental laws of physical dynamics are reversible then conceptually any machine should be able to run the laws of physics backwards and thus be able determine the system's backward states.   
 
% thus, non-reversible computation leads to bit erasure/heat 
Specifically, Landauer observed the direct implications on the thermodynamic behaviour of a device that is carrying out irreversible operations. His reasoning can be understood by realising that reversibility at the lowest level of physics means that we can never truly erase information in a computer. He notes that for the entire history of computers our computing machines have been erasing bits of information in the process of performing irreversible computations. 

If we return to the example of the logic gate AND, we can observe that given the output 0, the input 1 has been erased after the execution of the operation. Whenever a bit of information gets overwritten by a new value or whenever a logic gate  produces several unused outputs, the previous information might get lost but it will not be physically destroyed. Instead, bit erasure pushes bits out into the computer's thermal environment, where they become entropy causing heat dissipation and, in general, loss of energy. This is known as the von Neumann-Landauer (VNL) principle~\cite{maxwell} where one bit's worth of lost logical information always leads to at least  $kTln2 $ ($k$ is the Boltzmann constant which is approximately $1.38	\times10^{-23}$ $J/K$, $T$ is the temperature of the heat sink in kelvins, and $ln2$ is the natural logarithm of 2 which is approximately 0.69315) amount of physical energy dissipation. 

This result is of great interest because it makes plausible the existence of thermodynamically reversible computers which could perform computations while dissipating considerably less energy per logical step. The energy used in reversible bit operations can be fully recovered and reused for subsequent operations so that every computation can be performed without bit erasures.  This means that a computation is physically reversible when it can be carried out without loss of energy or, more formally, with no increase in physical entropy and is thus energy efficient.


%we are reaching landauers limit 
Landauer's theoretical lower bound has since been experimentally confirmed and it has been argued many times that efficient operations of future computers require them to be reversible. In the scenario of low-energy computing, the gap between computation and reality needs to be bridged by introducing the reversible or possibly the quantum mechanical  mode of computation. Currently, computers are commonly irreversible with their technology rapidly approaching the  elementary particle level extrapolating towards Landauer's limit. 

In particular, based on Moore's law, computer power roughly doubles every 18 months for the last half century~\cite{TimeSpaceBound}. The miniaturisation of  transistors increases their per-area leakage current and standby power; meanwhile, the reduction of signal energies, causes significant  thermal fluctuations  which eventually prevent any further progress within the traditional computing paradigm~\cite{back}. Efforts are being made within the semiconductor industry to try to reduce and forestall these problems, but the solutions are becoming ever more expensive to deploy where eventually no level of spending can ever defeat the laws of physics. Smaller transistors in new conventionally-designed computers would no longer be any cheaper, faster, or more energy-efficient than any predecessors, and at that point, the progress of conventional semiconductor technology will stop being any longer economically justifiable. In figure \ref{Landauer} we can see that landaure's limit threatens to end improvements in practical computer performance within the next few decades and to avoid this a solution could be to avoid losing track of logical information.

\begin{figure}[t]
\centering
\subfigure{\includegraphics[width=13cm]{figures/landauerslimit}}
\caption{Landauer's Limit}
\label{Landauer}
\end{figure}

%Save info
%Save every input
However, for several decades now, we have known that reversible computing is a theoretically possible alternative paradigm which is in fact the only possible way, within the laws of physics, to have energy and cost efficient computers. Although, when reversible computations are implemented on the right hardware, they should be able to circumvent Landauer's limit.  Lecerf~\cite{lecerf} was the  first to describe reversible computations executed on reversible Turing machines, and invented the Lecerf reversal technique to uncompute histories, but he was unaware of Landauer's thermodynamic applications, and  therefore his machines did not save their outputs. Bennett~\cite{Bennett} then reinvented Lecerf's  reversal based on Landauer's point of view that any desired logically irreversible computational operation could be embedded in a reversible one, by simply saving aside any information that it would otherwise erase. For example, the machine might be given an extra tape to record each operation as it was being performed, in order to be able to uniquely determine the preceding state by the present state and the last record on the tape. However, Landauer noted that this method was only going to postpone the inevitable, because the tape would still need to be erased eventually, when the available memory filled up. 

%Bennett
Bennet managed to prove that it is possible to construct fully reversible Turing machines capable of performing any computation whilst erasing garbage information on its tape when it halts and therefore leaving behind only the desired output and the originally furnished input. The trick is to decompute the operations that produced the intermediate results and therefore erasing the temporary data from the memory. This would allow any temporary memory to be reused for subsequent computations without ever having to erase or overwrite it. He also pointed out the possibility of a physically reversible computer where dissipation of energy is arbitrarily small. 

%Toffoli
However Bennett's construction only addressed the logical level where any arguments based on thermodynamics needed to be applied on specific hardware technologies.  Toffoli and Fredkin~\cite{FredkinToffoli} were the first to address precisely how to construct a practical physical mechanism for computation that would also be physically reversible. They have reinvented reversible computing in the form of conservative logic circuits, and proved their universality. Toffoli~\cite{Toffoli} invented the Toffoli gate which is perhaps the most convenient universal reversible logic primitive. All these pioneering developments together incrementally set the stage for the field of reversible computing.

% RC gives minaturization, less heat, more energy
Therefore, reversible computing has potential to alleviate the ever-increasing demand for electricity by designing revolutionary reversible logic gates and circuits that lead to low-power computing. Hardware-wise, the potential benefits of reversible computing come to solve the miniaturisation limitations of current technology that aim to increase the speed and capacity of circuits. On the other hand, there already exist various occasions where reversibility is naturally embedded in computation. For example, recovery from failures such as corrupted data, deadlocked programs and breached security is crucial and could be effortlessly obtained in a reversible manner.  Hence, such a mode of computation aligns naturally with many computational tasks such as the treatment of fault tolerance and recovery in distributed systems, coding and decoding and many others. 

%limitations 
So far, it is considered to be highly challenging to implement reversibility effectively, because it comes with many underlying problems and the alternative of advancing conventional technology is much easier. Even though it comes with many promising benefits and applications it also comes with its own limitations. Since, the theory of Reversible Computation is based on the idea of computing and uncomputing operations, it means that arbitrarily large computations executed in reverse would result in almost twice as many steps as an ordinary computation and may require a large amount of temporary storage. This means that there is an underlying trade-off between the efficiency of such recovery and the speed of computation.  

On a practical level achieving efficient reversible computing will likely require new hardware materials, new design tools and device structures, new hardware description languages with the supporting softwares and overall a thorough remodelling of the entire computer design infrastructure. This also means that a large part of computer scientists and digital engineering workforce will have to be trained to use novel reversible design methodologies.

Nevertheless, the upside potential of reversible computing has attracted many researchers that made significant conceptual progress over the past few decades. This effort of addressing the challenges of reversible computation is highly worthwhile, because with the current rapidly advancing technology, it is now time to focus on reversible computing, and begin collaborative effort to materialise this idea. Committed attention can eventually improve current information technology by making it many orders of magnitude greater than any existing irreversible technology. 

\subsection{Current State of Knowledge}
%RC is usefull in mary application areas
Computer Scientists, mathematicians and physicians believe that Reversible Computation will be a key technique in the not so distant future of computer models. It is generally believed that in 10 to 15 years all computers will be reversible since this very promising technology, that suggests that computation can run backwards as natural as it can go forwards, essentially leads to low power computing and hardware. Reversible computing attracts much interest for its potential in a growing number of application areas ranging from cellular automata, software architectures, reversible programming languages, digital circuit design to quantum computing. 

 
\subsubsection{Models of Computation} 
There exist several notions of logical  reversibility  on computing models with a finite number of discrete internal states that evolve in discrete time. Their precise impact on the computational capacities and decidability properties of devices has been considered from different points of view. In the literature there exist various models, including the massively parallel model of cellular automata, the weakly parallel model of multi-head finite automata as well as sequential models as Turing machines, pushdown and queue automata, and finite state machines. 

In order to examine whether reversibility increases computational capacities it is useful to study the properties and the impact on suitable models when different notions of reversibility are applied. These models have been equipped with additional resources or structural properties in order to examine whether a computational model can be made reversible and the associated costs. 

There have been proposals for reversible finite-state machines with additional storage, such as pushdown stores~\cite{RPA}, input-driven pushdown stores~\cite{inputDriven} and queues~\cite{queue}.  On the opposite end of the spectrum, there are reversible finite-state machines that do not use any additional resources~\cite{minimal}. %Additionally, in ~\cite{91} cellular automata that have discrete internal states have been studied for the first time.

 As mentioned before one of the fundamental studies produced by Bennett~\cite{Bennett} concerns the standard universal computational model of Turing machines. He proposed an efficient reversible simulation that demonstrates that any computation executed on Turing machines can be simulated reversibly. In general, reversibility is considered to be expensive because of the interplay between the increase of computational complexity and resources. Although~\cite{tapeReduction} has shown that tape reduction of reversible Turing machines can be done with no additional cost with respect to this resource. 
 
On the other hand, when it comes to multi-head reversible automata  restricting the space available leads to a separation between irreversibility and reversibility. Reversible computation in multi-head or finite automata  can be divided to one-way head motion~\cite{oneWay,RA} versus two-way~\cite{multiHead,twoWay}. %and reversible on all states versus reversible on reachable states. 

\begin{figure}[h]
\centering
\subfigure{\includegraphics[width=14cm]{figures/Automaton}}\\
\caption{Construction of a reversible automaton accepting $\langle a\overline{b}a, abba\rangle$~\cite{pin1992reversible}}
\end{figure} 


\subsubsection{Programming languages } A number of interesting reversible programming languages have been developed since 1986. The main challenge here is that these languages are still prototype languages. Thus, the code base for each of these languages is limited, and the languages do not offer many of the usual programming abstractions. This in turn has hindered the developments of reversible algorithms and useful data structures. Reversing the state of a system might mean going back to an earlier version of its state. The cost of storing previous versions of large data structures can be prohibitive. Persistent (immutable) data structures~\cite{DataStructures} offer more efficient storing of multiple versions of a data structure, sharing structure where possible. %This makes it possible to simply store previous state information without excessive memory pressure.  Reversible flowcharts have also been proposed that are equipped with an assertion operator which can be simulated by a structured reversible flowchart using only three control flow operators~\cite{Flowchart} .

 The first reversible programming language that follows the imperative paradigm, named Janus,  was created by Lutz~\cite{Janus}, and it has later been `rediscovered', formalised and further developed in~\cite{ Flowchart}. Another simple reversible imperative languages is R~\cite{R}. 
 
\begin{figure}[h]
\centering
\subfigure{\includegraphics[width=14cm]{figures/Flow1}}\\
\caption{Structured reversible control flow operators~\cite{Flowchart}}
\end{figure} 

\begin{figure}[h]
\centering
\subfigure{\includegraphics[width=14cm]{figures/Flow2}}\\
\caption{Inverted structured reversible control flow operators~\cite{Flowchart}}
\end{figure} 
% and several reversible machine languages, such as PISA and BobISA. 
Reversible functional programming has also been attracting interest starting from 1996 when Huelsbergen presented an evaluator for the lambda calculus named SECD-H~\cite{SECDH}. Other general purpose functional programming languages are RFUN~\cite{RFUN}, muOz~\cite{muoz} the causal-consistent reversible extension of Oz and Theseus~\cite{Theseus}. One of the advantages of reversible functional languages is that they support more complex data types than those of the reversible imperative languages, which have been limited to integers, arrays and stacks.

Reversibility is also related to quantum computing, since quantum programs are always logically reversible. The first family of quantum programming languages consists of languages based on the imperative paradigm. QCL (Quantum Computation Language)~\cite{QCL} is one of the most advanced quantum programming languages with working interpreter, followed by LanQ~\cite{LanQ}. The second family of quantum programming languages consists of languages based on the functional paradigm. One of these functional quantum languages is cQPL~\cite{cQPL} which has classical elements similar to those implemented in imperative programming languages. QML is another quantum programming language following a functional paradigm developed by Altenkirch and Grattage~\cite{QML}.
 
Research on compiler technology for reversible languages has also progressed in the last several years. One can now translate reversible high level languages to reversible machine code. The first compiler between R and PISA was made by Frank~\cite{R}. The most notable developments are the Janus compiler~\cite{Translation}  and was clean in the sense that the compiled program did not have more than a constant memory overhead over the original Janus program. The key insight here is that translations must be clean and incur no garbage overhead. This requires novel insights and solutions which are absent in the irreversible programming languages setting.


\remove{
\subsubsection{Process calculi } 

Research on process calculi traces back to~\cite{abstract}, which is a calculus inspired by biochemistry whose operational semantics are able to model both forward and backward chemical reactions.  Although, the first reversible reformulation of already existing process calculi dates back to  RCCS~\cite{RCCS,BiologyCCSR} a causal-consistent reversible extension of CCS~\cite{ccs} that  uses memory stacks in order to keep track of past communications, further  developed  in~\cite{TransactionsRCCS}.  The main contribution of their work is the notion of causal-consistent reversibility. In the scenario of concurrent or distributed systems,  backward determinism is too restrictive since it only allows reversal of the last executed action.  They introduce the relation between reversibility and causality instead of time, which in the case of distributed systems means that actions are allowed to reverse as long as their effects ( or caused actions) are not executed or they have been reversed~\cite{causality}. 


A general method for reversing process calculi was subsequently proposed in~\cite{Algebraic}
with CCSK being  a special instance of the methodology. This proposal introduces keys to bind synchronised actions together. Constructs for controlling reversibility were also  proposed  in reversible extensions of the $\pi$-calculus in~\cite{LaneseLMSS13,LaneseMSS11,LaneseMS16,DBLP:conf/lics/CristescuKV13}, where the authors rely on  simple thread tags, which act as unique identifiers. Most recently, the study of out-of-causal-order  reversibility continued with the introduction of a new operator  for modelling local reversibility in~\cite{LocalRev}.  

The study of reversible process calculi triggered also research on more abstract models for describing concurrent systems such as event structures~\cite{ConRev}. The modelling of bonding within reversible processes and event  structures was also considered in~\cite{ Bonding}, whereas a reversible computational calculus for modelling chemical systems, composed of signals and gates, was  proposed in~\cite{CardelliL11}. Reversibility has also been extended to Quantum process calculi, that are used to describe and model the behaviour of systems that combine classical and quantum communication and computation the most prominent being qCCS ~\cite{qccs} and CQP~\cite{cqp}. 

\begin{figure}[h]
\centering
\subfigure{\includegraphics[width=15cm]{figures/ProcessCalculus.png}}
\caption{Reversible Process Calculi~\cite{causality}}
\end{figure}

On another note, having models that express uncontrolled reversibility is of no use in real life applications. For instance, various biological phenomena control the direction of the computation based on physical conditions such as temperature, pressure and reaction rates.  Therefore various mechanisms for controlling reversibility in process calculus have been proposed. In particular, ~\cite{RCCS,sessionBasedPi} introduced irreversible actions in order to avoid reversing after a relevant result has been executed. Where, ~\cite{tuple,LaneseLMSS13,LaneseMSS11,compensations} have proposed an explicit rollback operator that allows the reversal of executed actions during forward computation, and a mechanism providing alternative paths. In ~\cite{ERK} , a forward monitor has been proposed in order to control the direction of execution of a reversible monitored process. Finally, a local mechanism was introduced in~\cite{LocalRev} where an amount of executed actions needs to be reversed  in order to be able to perform new forward actions. 

Reversible calculi were born  with mainly biological motivation. Since many biological phenomena are naturally reversible, a reversible formalism seems to be suitable to model such systems. Indeed, efforts have been made to model biological systems~\cite{CardelliL11,BiologyCCSR,ERK,Bonding} as well as chemical reactions~\cite{LocalRev} using reversible process calculi. We highlight~\cite{CardelliL11} which illustrates a compilation from asynchronous CCS to DNA circuits.

\begin{figure}[h]
\centering
\subfigure{\includegraphics[width=6cm]{figures/RPC.png}}
\caption{Reversible Process Calculi for biological systems}
\end{figure}

Given their formal definition, process calculi are suitable to formally verify properties of systems. There is a strong line of work concerned with applications of reversible process calculi such as Session types and contracts, biological phenomena, constructs for reliability.  ~\cite{sessionBasedPi} shows how the session type discipline of $\pi$-calculus extends to its reversible variants. In~\cite{singleSessions}, (binary and multiparty) session type systems are used to restrict the study of reversibility in $\pi$-calculus to single sessions. Instead, ~\cite{ServerClient,retractable} study the compliance of a client and a server when both of them have the ability to backtrack to past states.

In a different setting, reversible process calculi have also been used to build constructs for reliability, and in particular communicating transactions with compensations~\cite{Kutavas}. Transactions with compensations are computations that either succeed, or their effects are compensated by a dedicated ad-hoc piece of code. In~\cite{Kutavas}  the effect of the transaction is first undone, and then a compensation is executed. Behavioural equivalences for communicating transactions with compensation have also been studied  in~\cite{Kutavas2,Kutavas3}. In~\cite{LaneseLMSS13} interacting transactions with compensations are mapped into a reversible calculus with alternatives.
}

\subsubsection{Reliable software } 

The idea of using reversibility for the development of reliable software is quite natural since  backward recovery is an instance of reversible computation in which errors trigger inverse actions. When a failure occurs in a system it means that the behaviour of the systems differs from the behaviour that has been previously specified. Fault tolerance comes to aid such system failures by eliminating the presence of faults and therefore providing  the required level of service from a system that is highly dependable. As in figure \ref{GDB}, in case of trouble fault treatment seeks to handle certain system errors after their occurrence and therefore stop them from causing a failure. Then the system can go backwards to a past safe state of the system and try to explore new directions, avoiding the troublesome actions and therefore bringing the system to a consistent state.  

Reversibility provides a high-level setting for examining and ultimately specifying, and verifying fault tolerant systems with backward recovery. %For instance, in distributed systems, checkpointing allows recovery of previously saved states that are safe from errors where transactional recovery reverses their effects in case of abort.
 If a fault is detected, checkpointing can be used as recovery mechanism that restores the system to a previously saved state which is essentially a snapshot of the entire system that is safe from errors. In~\cite{RevComProc} a reversible extension of the Scala language supporting channel-based synchronisation is presented. Whereas, ~\cite{Transactors} proposes a fault tolerant programming model for composing loosely-coupled distributed components that use the checkpoint-recovery technique in the actor model. %It extends the actor model with constructs which distributed processes can use to to build globally consistent distributed checkpoints. 
\cite{ML} proposes Stabilisers which is a concurrent ML language for transient concurrent fault recovery %in concurrent program
 which is able to deal with program global checkpoints. %The language introduces three new primitives: stable, stabilise and cut, able to deal with program global checkpoints. %Transactors: a programming model for maintaining globally consistent distributed state in unreliable environments
 
The past 40 years reversibility has also been naturally applied in the area of  debugging~\cite{AIDS,RevEx} because it gives the ability to explore the computation in both forward and backward, and therefore assisting the programmer in the search of possible misbehaviours. Standard debuggers require the programmer to restart the execution and put a breakpoint where one thinks the error causing it is. Whereas, in reversible computation when a bug is found, the programmer can simply retrace back his steps in the execution till the error causing it has been found. 

Reversibility for debugging of sequential programs has been quite extensively explored. Indeed, many reversible debugging tools exist ~\cite{RevDeb,Igor,RevDebugger,Java} and some reversible debugging features are available in mainstream debuggers for instance even GDB supports reversible debugging since version 7.0. So far in order to enable reversible debugging strategies, one has to keep track of past history, and the related overhead required to store history information both in terms of time and in terms of space may be heavy, which makes the use of reversible debuggers for large programs fairly difficult. Keeping history information and consistent reduction of the heavy overhead is still a very challenging open problem when it comes to debugging. However, at the industrial level there exist some state of the art techniques based on incremental storage of information and complex fine tuning that allow overhead reduction.% [136].

\begin{figure}[h]
\centering
\subfigure{\includegraphics[width=11cm]{figures/Debugging}}
\caption{GDB reverse Debugging}
\label{GDB}
\end{figure}

\remove{
In a sequential setting reversibility is very natural because steps are recursively undone in the exact reverse order of execution. Although, in the concurrent setting there is no clear last executed action since many actions can be executed at overlapping times and therefore %Although nowadays, most systems are composed of many concurrent and possibly distributed entities%: computers in a network, processors in a computer, cores in a processor, threads, and so on. 
reversibility has been defined as a causal-consistent reversibility back in 2004~\cite{RCCS}. According to causal-consistent reversibility, any action can be undone, provided that all the actions causally depending on it, if any, are undone beforehand. This definition relates reversibility to causality instead of time, thus allowing one to exploit it even if there is no unique notion of time for all the participants, as it may happen in distributed systems. 
}

The definition of causal reversibility has spawn various reversible extensions of concurrent languages that are used for validating formal connections between causal-consistent reversibility and reliability as well as studying its consequences. It enables a new strategy for debugging concurrent systems, where the different speed of processes that are replaying an execution looking for a bug may cause different behaviours.%, and even eliminate the misbehaviour one was trying to analyse. 
There have been proposed reversible process calculi used to build constructs for reliability, and in particular communicating transactions with compensations~\cite{Kutavas} where interacting transactions with compensations have been mapped into a reversible calculus with alternatives in~\cite{LaneseLMSS13}. ~\cite{Kutavas} uses transactions with compensations, which are computations that either succeed, or their effects are reversed and then a compensation is executed by a dedicated ad-hoc piece of code. %In relation to reliability, formal connections between causal-consistent reversibility on one side, and transactions and rollback on the other side, have been made. 
The behavioural equivalences for communicating transactions with compensation have been studied in~\cite{Kutavas2,Kutavas3}. 

\subsubsection{Control Systems and Robotics } Robots are generic mechatronic devices controlled by a computer that can essentially be made reversible. Reversibility plays vital role in different programming paradigms that are used to operate robots. The area of control systems and of robotics can benefit from reversibility depending on the type of robot. %. Given the massive diversity in robotic machinery, the meaning of robotic reversibility is likely to depend on the type of the robot, and is not necessarily meaningful for all kinds of robots. 

In control systems, reversibility can be applied in %an interesting application concerns
systems that can autonomously accumulate and revise knowledge from their own experience via self-programming. Control systems operate concurrently during forward execution in order to predict the behaviour of the environment under constrains of limited time and computational resources. Whereas, during backward execution they retrieve the goals the system was designed to achieve. %Forward and backward executions of models are performed concurrently and their goodness is measured based on the quality of the predictions they make about the behaviour of the environment relative to the goals the system was designed to achieve. 
 
 Reversibility in robot programming languages was first made in the context of modular robotics which is an approach that uses a reconfigurable assembly of simple subsystems. % ~\cite{131}.
Modular components use self-reconfiguration to achieve flexibility and reliability by being able to rearrange modules automatically and only where necessary. Self-reconfiguration is a reversible process and it has been investigated in the ATRON  modular robot ~\cite{SelfReconfig} (shown in Figure \ref{ATRON}). A more general reversible language that is used for programming such modular robot systems is $\mu$rRoCE (micro reversible robust collaborative ensembles)~\cite{murRoCE}.

% n%A sequence is specified using a simple, centralized scripting language named DynaRole. Dyna- Role programs could be manually written or automatically generated by a planner. 
 %an effort to provide a more general reversible language for controlling modular robots, the languagewas devised as a minimalistic, general-purpose and reversible language for programming modular robot systems [124].  
 
%but it can be affected by physical constraints such motion limitations and changes in the environment. Schultz et al investigated the distributed execution of a pre-specified self- reconfiguration sequence 

\begin{figure}[h]
\centering
\subfigure[Cluster]{\includegraphics[width=5cm]{figures/Cluster.png}}
\subfigure[Car]{\includegraphics[width=5cm]{figures/Car.png}}
\subfigure[Snake]{\includegraphics[width=5cm]{figures/Snake.png}}
\caption{ATRON modular robot~\cite{Brandt2007ATRONRV}}
\label{ATRON}
\end{figure}

Many operations in the field of robotics are naturally reversible both for single robots as well as multi-robot swarms. These operations include reversing the forward execution of an assembly sequence in order to generate the backward disassembly process as well as changing the direction of a mobile robot from forward to backward. % Clearly, the interplay with non-reversible actions needs to be taken into account. Thus, reversibility may allow one to have for free useful reverse behaviour, or also new interesting emerging behaviours. Industrial robots are increasingly being used for complex operations like assembly of products. 
 The increase likelihood of errors in industrial robots % increases with the complexity of the assembly operation %. As an extension to the standard use of reversibility for debugging (see also Section 3.4), it has been proposed that certain classes of errors during assembly operations and
can be addressed using reverse execution in order to withdraw an erroneous situation and thereafter automatically retry the assembly operation~\cite{ErrorRecover}. The assembly sequence can be programmed in  RASQ~\cite{RASQ}, which  is a reversible DSL  that whenever an error is encountered  it automatically derives a disassembly sequence in order to recover the assembly sequence.


\subsubsection{Reversible circuit design} 
As motivated  by Lundauer~\cite{Landauer}, reversible circuits  have several promising applications such as low-power circuit design and quantum computing. The inherent properties of reversibility can be exploited in the design of conventional circuits with many advantages. One of them is the ability to undo operations in case the system reaches an erroneous state as well as full connectivity which detects errors by applying randomly generated stimuli. Conventional computing also benefits from reversibility by achieving perfect observability and controllability which provides easy testability.  

Another application of reversible circuits is quantum computing~\cite{QuantumComputing} which is inherently reversible and allows reversible computation to be exploited as a subset of quantum operations. The applied encoders in quantum computing already generate reversible one-to-one mappings that enable the synthesis of reversible logic gates. Reversibility also benefits quantum computing with low-power interconnects that decrease the overall energy consumption in chips. % With the rise of very deep sub-micron and nano-metric technologies, interconnects are increasingly affecting the overall energy consumption in chips.
% As a result, coding strategies are applied in order to modify the communication of interconnects and, thus, reduce the power consumption. Since the applied encoders realise reversible one-to-one mappings, the application of synthesis approaches for reversible logic is a reasonable choice. 

The goal of conventional circuit design is to find a logic circuit that implements the Boolean function and minimises the number of gates or the circuit depth.  Reversible circuit synthesis is a special case of conventional circuit design where all gates are made reversible by disallowing any fanout. In order to avoid any fanout, it must be that the number of input wires of a gate is the same as the number of output wires. Therefore, there is an one-to-one mapping between inputs and outputs allowing the input states to be reconstructed from the output states~\cite{regular}. Each gate can be made reversible by adding some additional input and output wires if necessary~\cite{QuantumComputing} and therefore being able to uniquely recover any input from a given output.  

The most well known gates in reversible and quantum computing are the Fredkin gate~\cite{fredkin} (Figure \ref{Gates} (c)) together with Toffoli~\cite{Toffoli}  (Figure \ref{Gates} (a)) and Feynman~\cite{feynman} (Figure \ref{Gates} (b)) gates. The Fredkin gate is a universal circuit with three bit inputs and three bit outputs where the first bit is transmitted unchanged and the last two bits are swapped if, and only if, the first bit is equal to 1. The second universal gate, called the Tofolli gate, is also known as the "controlled-controlled-not" gate, which describes its action. Similarly to Frdkin gate, Toffoli also has three inputs and three outputs where the third bit is inverted if the first two bits are both set to 1, otherwise all bits stay the same. The Fyenman gate also has three bit inputs and three bit outputs where two of the inputs are transmitted unchanged and the third input is also transmitted unchanged unless the other two inputs are both 1, in which case the third bit is inverted.  

\begin{figure}[h]
\centering
\subfigure[Toffoli]{\includegraphics[width=4.8cm]{figures/Toffoli.png}}
\subfigure[Feynman]{\includegraphics[width=4.5cm]{figures/Feynman.jpg}}
\subfigure[Fredkin]{\includegraphics[width=5.4cm]{figures/Fredkin.png}}
\caption{Reversible Logic Gates}
\label{Gates}
\end{figure}


